Unit Grid Intersection Graphs: Recognition and Properties

It has been known since 1991 that the problem of recognizing grid intersection graphs is NP-complete. Here we use a modified argument of the above result to show that even if we restrict to the class of unit grid intersection graphs (UGIGs), the recognition remains hard, as well as for all graph classes contained inbetween. The result holds even when considering only graphs with arbitrarily large girth. Furthermore, we ask the question of representing UGIGs on grids of minimal size. We show that the UGIGs that can be represented in a square of side length 1+epsilon, for a positive epsilon no greater than 1, are exactly the orthogonal ray graphs, and that there exist families of trees that need an arbitrarily large grid.

==> clause.tex <==
\input epsf
\epsfbox{obrazky.4}

\epsfbox{obrazky.6}

\epsfbox{obrazky.7}

\epsfbox{obrazky.8}

\bye


==> offsets.tex <==
\DeclareGraphicsRule{.6}{mps}{*}{} 
\DeclareGraphicsRule{.7}{mps}{*}{} 
\DeclareGraphicsRule{.8}{mps}{*}{} 
\DeclareGraphicsRule{.9}{mps}{*}{} 
\DeclareGraphicsRule{.11}{mps}{*}{} 
\begin{prop}
Any unit grid intersection graph on $n$ vertices can be represented
in a grid $(n+1)\times (n+1)$ with all coordinates being multiples
of $1\over n$. Moreover, we can find such a representation that
with respect to a particular axis no two segments have the same
non-integral part of the coordinate.
\end{prop}

Note that the lower bound (multiples of $1\over n$) is tight because
of $K_{1,n-1}$ which requires this precision for the coordinates.

\begin{proof}
Let us consider an arbitrary UGIG-representation of a given graph. We
proceed for each axis separately (for each axis we find
a canonical representation). Considering an appropriate projection
onto (without loss of generality) $x$-axis, we obtain the arrangement of unit
intervals and points (representing the orthogonal intervals). Let us consider
a representation in general position, i.e., no two endpoints are
the same and also individual points do not coincide with, neither
each other, nor with other endpoints.

To simplify the following sweeping-argument, we extend individual points
to unit-segments (in arbitrary fixed direction). So we obtain
an arrangement of unit segments. Now we perform the sweep: Starting
from the right to the left, we start building canonical representation.

For the right-most segment let us take the representation where the
left endpoint lies on coordinate $0$. The so far built canonical
representation gets completely rebuild when adding a new segment $s$.
What we do (while adding the new segment) is that we shift the
representation in such a way that the endvertex $t$ lying as the next
to the right from the right end-vertex of $s$
lies on an integral coordinate (we shift the representation
by $k\over m$ where $m$ is number of so far represented segments).
After this shift we create the space for segment $s$
in the following way: Coordinate $k+{l\over m}$, where
$k, l$ and $m$ are integers, $l$ and $m$ are non-negative
($m$ is the number of so far
represented segments), change to $k+{l+1\over m+1}$. In this way
we modify the whole (so far
existing) representation. Before this transformation the endpoint
$t$ had the coordinate $u$. After the transformation the endpoint's coordinate
is $u+{1\over m+1}$. We represent the right endpoint of $s$ on coordinate
$u$ (and the left on $u-1$). In this way we obtained the appropriate
place for the right endpoint. The left endpoint is represented correctly
because we are sweeping from the right to the left and thus the newly added
segment's left-endpoint is the leftest in so far built arrangement.

When the sweeping process finishes, we have the canonical representation.
Now it suffices to shrink unit-segments representing perpendicual segments
back to one point. Their extending was a technical point avoiding us to
decide whether the individual points should behave similarly to left-
or right-endpoints. Note that the algorithm assigns to the newly-added
segment the non-integral part different from all the others and that
when shifting the representation,
we are shifting the whole representation (thus different non-integral
parts remain different) and the process of "making space for the new
segment" also maps different non-integral parts to different values.
Thus at the end of the process no two segments have the same non-integral
part in the assigned coordinate.

This shows the lower bound (i.e., that we do not need smaller precision
than $1\over n$), as well, as assigning different non-integral parts.
What remains is an upper bound. This gets done by the following observation:
When does the canonical representation grow and by what factor? This
growth must be caused by the newly-added segment and the highest growth gets
caused by a segment disjoint with all so far represented segments. In this
way we extend the representation by 1 and some fraction (that gets changed). 
After adding $n$ segments, this fraction (for each added segment) is $1\over n$.
As this blow-up can take place with each segment, together we can bound
the size (from above) by $n+1$ (more precisely it is $n+{n-1\over n}$).

Note that the upper bound is visibly not tight (because the worst
counterexample comes from a stupid representation of a graph with no
edges). Also note that this construction for canonical representation
works also for not necessarily
unit segments but also for general axis-aligned segments (the sweep
would be done with respect to
the left endpoint of individual intervals and it would be necessary
to recalculate the upper bound on the size of the underlying grid).

\begin{figure}
(a) \includegraphics{obrazky.6}    (b)\includegraphics{obrazky.7}
\hfill (c) \includegraphics{obrazky.8}  \\
\hrule
  (d)\includegraphics{obrazky.9}
\hfill (e) \includegraphics{obrazky.11}
\caption{Considering the arrangement from picture (a) we make a projection onto one axis (b), i.e., perpendicular segments collapse into single points. We extend them in one direction (in our case to the left), see picture (c). Picture (d) shows the fourth step of the sweeping algorithm, i.e., extending so far obtained representation. Picture (e) shows the final representation (with respect to $x$-axis, to obtain the desired representation it would be also necessary to sweep along the $y$-axis).}
\end{figure}

\end{proof}


==> section4.tex <==
 This section will be dedicated mainly to proving the following
 \begin{thm}\label{thm:nphard}
It is NP-hard to distinguish whether a given graph has a UGIG-representation
or whether it does not even admit a representation by pseudosegments. Considering
any constant $k\in \mathbb{N}$ this holds even when restricting the analysis to graphs of girth at least
$k$.
\end{thm}
\begin{cor}
The recognition problem is NP-hard for any class containing UGIGs
which is simultaneously contained in class of pseudosegment-graphs. For
such a class the recognition problem remains NP-hard even if restricted
to graphs with arbitrarily large girth.
\label{dusl:jednoduchy}
\end{cor}
\begin{cor}
The recognition problem is NP-complete for UGIGs as well as for
USEG graphs and the property holds even when
restricted to graphs with arbitrarily large girth. \label{dusl:npcompleteness}
\end{cor}


Because of the page-limit, we only sketch the proof here. The full version of this
section can be found in the Appendix. As the proof uses a similar reduction to \cite{KP},
we focus mainly on the difference. The reduced problem is that of planar 3-connected
3-SAT(4). A clause gets encoded by the clause gadget, variables get encoded by
the variable gadget and the occurences by occurence gadgets, respectively. The
"occurence gadget" is just a pair of paths (as in \cite{KP}). It can clearly be represented and it does the same job. The clause gadget is also
the same (it is only necessary to show that it has a unit grid representation for suitable truth assignments) - see Figure \ref{clause:gadget}.

\begin{figure}[htbp]
\begin{minipage}[b]{0.3\linewidth}
\centering
\includegraphics[width=4.5cm]{obrazky.19}
\end{minipage}
\begin{minipage}[b]{0.7\linewidth}
\centering
\includegraphics[width=8cm]{oneinstance.pdf}
\end{minipage}
\caption{Left: the clause gadget. Right: UGIG representations for the clause gadget for two suitable truth assignments, TTT and TFF, respectively (the outer cycle is not represented)}
\label{fig:instance}
\end{figure}


%PerM: Here we could insert [into the same raw] at least onw and at most
%two representations.
\begin{figure}[h]
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=3cm]{obrazky.1}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=3cm]{obrazky.2}

\end{minipage}
\label{variable}
\caption{The variable gadget: true(on the left) and false (on the right) assignment}
\end{figure}


What is innovative, is the variable gadget that does not require the cross-over
gadget. Such a variable gadget (for four occurences) is depicted in Figure
\ref{variable}. Note that it preserves the left-right orientation of the pairs
of paths stemming from the cross for any representation up to
pseudosegment-graphs whenever there are four occurences (and whenever these
occurences stem from the center in a prescribed ordering -- which is ensured
by 3-connectivity of the graph corresponding to the formula). We are guaranteed
(by the problem) that each variable appears at most 4 times and 3-connectivity
also ensures that each variable appears at least 3-times. Whenever a variable
has only 3 occurences, we have to adjust the variable gadget by introducing a "dummy
occurence" to keep the left-right orientation consistent. This gets done
by the "dummy-gadget" depicted in Figure \ref{dummy:occurence}. As this
graph is either representable as a UGIG or not representable even as a PSEG,
the hardness part of the Theorem \ref{thm:nphard} follows.

\begin{figure}[htbp]
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=4cm]{obrazky.21}
\end{minipage}
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=4cm]{obrazky.20}
\end{minipage}
%PerM: We should make the caption a bit more precise (the representation lacks the details inside the circle:
%\caption{A dummy gadget (left) with an appropriate UGIG representation (right).
%}
\caption{A dummy gadget (left) with an appropriate UGIG representation (right). Note that in the representation we omitted the details inside the circle where
the paths should be appropriately connected to segments representing $a$ and $b$.}
\label{dummy:occurence}
\end{figure}

Now we show the remaining part of the proof of Corollary \ref{dusl:npcompleteness}. Although we could use the canonical construction with Cartesian coordinate-system, as we are interested in optimal representations, we show that even a simpler certificate suffices:

\begin{thm}
 The recognition problem for  UGIG and USEG graphs is in NP, i.e.,
there exists a certificate of size $O(n\log n)$ for which we can verify (in polynomial time) that it witnesses the representation.

\end{thm}


\begin{proof}
%PerM: Added a brief comment instead of the whole proof.
We use a method similar to the proof of equivalence between unit interval
graphs and proper interval graphs. We therefore proceed by encoding the ordering of start- and end-points for individual segments with respect to individual axes, with the remaining details being in the Appendix. %I deleted a sentence, it can all be seen in the Appendix
\end{proof}


